CODECLEANER: Elevating Standards with A Robust Data Contamination Mitigation Toolkit

Data contamination presents a critical barrier preventing widespread industrial adoption of advanced software engineering techniques that leverage code language models (CLMs). This phenomenon occurs when evaluation data inadvertently overlaps with the public code repositories used to train CLMs, severely undermining the credibility of performance evaluations. For software companies considering the integration of CLM-based techniques into their development pipeline, this uncertainty about true performance metrics poses an unacceptable business risk. Code refactoring, which comprises code restructuring and variable renaming, has emerged as a promising measure to mitigate data contamination. It provides a practical alternative to the resource-intensive process of building contamination-free evaluation datasets, which would require companies to collect, clean, and label code created after the CLMs' training cutoff dates. However, the lack of automated code refactoring tools and scientifically validated refactoring techniques has hampered widespread industrial implementation. To bridge the gap, this paper presents the first systematic study to examine the efficacy of code refactoring operators at multiple scales (method-level, class-level, and cross-class level) and in different programming languages. In particular, we develop an open-sourced toolkit, CODECLEANER, which includes 11 operators for Python, with nine method-level, one class-level, and one cross-class-level operator. A drop of 65% overlap ratio is found when applying all operators in CODECLEANER, demonstrating their effectiveness in addressing data contamination. Additionally, we migrate four operators to Java, showing their generalizability to another language. We make CODECLEANER online available to facilitate further studies on mitigating CLM data contamination.

==> Algorithm/Alg_code_decomposition.tex <==
\begin{algorithm}[t]
  \setstretch {1.00}
  \footnotesize
  \caption{Construct an Extended Loop/Call Graph}
  \label{alg:code_decomposition}
  \KwIn{The source code $C$ and the location $loc$ of the assertion to be verify}
  \KwOut{A call graph $G$ extended with loops}
  \BlankLine
    $G \leftarrow$ \texttt{get\_function}($loc$) ~\tcp*{\scriptsize initialize a Graph $G$}
    $WorkList$ $\leftarrow$ \texttt{get\_function}($loc$)\;
    \While{$WorkList != \emptyset$}{
        $Fn$ $\leftarrow$ \texttt{select\_and\_remove\_a\_node}($WorkList$) ~\tcp*{\scriptsize transitively visit all reachable nodes}
        \For{each basicBlock $bb$ in $Fn$}{ 
            \If(\tcp*[f]{\scriptsize If there exist a function call})
            {$bb$ calls a function $M$}{
                \If{$M$ is not already a node in $G$}{
                    Add a node $M$ to $G$\;
                    Add an edge from $Fn$ to $M$ in $G$\;
                    $WorkList$ $\leftarrow$ $WorkList$ $\cup$ $M$ ~\tcp*{\scriptsize Add this node (function) to the $WorkList$}
                }
            }
            \If(\tcp*[f]{\scriptsize If there exist a loop})
            {$bb$ is a loop entry for loop $L$}{
                \If{$L$ is not already a node in $G$}{
                    Add a node $L$ to $G$\;
                    Add an edge from $Fn$ to $L$ in $G$\;
                    $WorkList$ $\leftarrow$ $WorkList$ $\cup$ $L$ ~\tcp*{\scriptsize Add this node (loop) to the $WorkList$}
                }
            }
        }
    }
    \Return $G$ ~\label{algno:return_graph_end}
    % \vspace{-10pt}
\end{algorithm}

==> Algorithm/Alg_hierarchical_specification_generation.tex <==
\setlength{\textfloatsep}{0pt}
\begin{algorithm}[t]
  \setstretch {1.00}
  \footnotesize
  \caption{Hierarchical Specification Generation}
  \label{alg:specification}
  \KwIn{A loop/call Graph $G$, an iteration bound $t$, a Large Language Model $LLM$, and the assertion $ass$ to be verified}
  \KwOut{Annotated Code $C$ with generated specifications}
  \BlankLine
    $C$.\texttt{init}() ~\tcp*{\scriptsize initialize a code template} \label{algno:initg}
    \For(\tcp*[f]{\scriptsize iteratively enhancing specifications}){$i$ in \emph{\texttt{range}(0, $t$)}~\label{algno:iterate}}{
        Initialize a stack $S$ with the $root$ node of $G$~\label{algno:initstack}\;
        \While{$S$ is not empty~\label{algno:while_stack}}{
            $f$ = $S$.\texttt{top}() ~\tcp*{\scriptsize get the element at the top of the stack}
            $allgen$ = true\;
            \For{each $callee$ in $f$.\emph{\texttt{callees}()}~\label{algno:callee1}}{
                %\If{the specifications of $callee$ is not generated in this iteration~\label{algno:callee_gen}}{
                \If{ spec generation for $callee$ has not been done in $i^{th}$ iteration~\label{algno:callee_gen}}{
                    $S$.\texttt{push}($callee$) ~\label{algno:push}~\tcp*{\scriptsize push all callee into the stack} 
                    $allgen$ = false ~\label{algno:allgen_false}
                }
            }
            \If {$allgen$ == true~\label{algno:allgen_true}}{
                $spec_{tmp}$ = \texttt{spec\_generation}($C$, $f$, $LLM$) ~\label{algno:specgen}~\tcp*{\scriptsize query LLM to generate specification candidates}
                $spec_f$ = \texttt{spec\_validation}($C$, $spec_{tmp}$) ~\label{algno:validate}~\tcp*{\scriptsize specification validation}
                $C$.\texttt{insert}($spec_f$) ~\label{algno:insert}~\tcp*{\scriptsize insert the specifications into the code template}
                $S$.\texttt{pop}() ~\label{algno:while_end}~\tcp*{\scriptsize pop up the top element $f$ of the stack} 
            }
        }
        \If(\tcp*[f]{\scriptsize determine whether the whole verification task has been completed}){\texttt{spec\_validation}($C$, $ass$)~\label{algno:assert}}{
            \texttt{simplify}($C$) ~\label{algno:simplify}~\tcp*{\scriptsize eliminating redundant or unnecessary specifications}
            \textbf{break} ~\label{algno:break}
        }
    }
    \Return $C$ ~\label{algno:return_code_end}
\end{algorithm}

==> Code/annotated.tex <==
#include <limits.h>

/* 1. FUNC CONTRACT */
void swap(int *a, int *b) {
    // omitted
}

/* 4. FUNC CONTRACT */
void bubbleSort(int *array, int n) {
    int i, j;
    /* 3. LOOP INVARIANT */
    for(i = n - 1; i > 0; i--) {
        /* 2. LOOP INVARIANT */  |\label{code:loop-2}|
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

void main() {
    // omitted
    //@ assert \forall int i; 0 < i < 5 ==> array[i-1] <= array[i];
}

==> Code/case-spurious.tex <==
int main() {
  int x = -50, y;
  // |\ding{53}| Loop invariant by Code2Inv:   ( ( x <= -50 |$\mid \mid$| y > ( 0 - 0 ) ) && ( x == ( x + 0 ) ) ) |\label{line:code2inv}|
  // |\ding{52}| Ground truth loop invariant: (x < 0 |$\mid \mid$| y > 0)
  while( x < 0 ) {   
    x = x+y;
    y++;
  }
  //@ assert(y>0);
}

==> Code/case-study-1.tex <==
void swap(int *a, int *b) {
	int temp = *a;
	*a = *b;
	*b = temp;
}

void bubbleSort(int *array, int n) {
	if (n <= 0) return;
	int i, j;
	for (i = n - 1; i > 0; i--) {
		for (j = 0; j < i; j++) {
			if (array[j] > array[j+1]) {
				swap(&array[j], &array[j+1]);
			}
		}
	}
}

void main() {
	int array [N] = {10, 7, 9, ...};
	bubbleSort(array, N);
}


==> Code/case-study2.tex <==
#include <math.h>

int fun(int n) {
    double y = 0, i = 0;
    /*@
        loop invariant y == (\pow(2, i)) - 1;
        loop invariant i <= n;
    */
    while(i <= n){
        y = y + pow(2.0, i);
        i = i + 1;
    }
    return y;
}

==> Code/case-study3.tex <==
/*@
requires \valid(a) && \valid(b) && \valid(r); |\label{line:spec1}|
ensures \result == *a + *b + *r;|\label{line:spec2}|
assigns \nothing;|\label{line:spec3}|
*/
int add(int *a, int *b, int *r) {
    return *a + *b + *r;
}

==> Code/code-temp.tex <==
#include <assert.h> // include the header file for assert

void swap(int *a, int *b) {
	int temp = *a;
	*a = *b;
	*b = temp;
}

void bubbleSort(int *array, int n) {
	if (n <= 0) return;
	int i, j;
	for (i = n - 1; i > 0; i--) {
		for (j = 0; j < i; j++) {
			if (array[j] > array[j+1]) {
				swap(&array[j], &array[j+1]);
			}
		}
	}
}

void main() {
	int array [N] = {10, 7, 9, ...};
	bubbleSort(array, N);
}


==> Code/code-temp2.tex <==
#include <assert.h> // include the header file for assert

void swap(int *a, int *b) { // use pointers as parameters to swap the values
	int temp = *a;
	*a = *b;
	*b = temp;
}

void bubbleSort(int *array, int n) {
	assert(array != NULL); // precondition: array is not null
	assert(n >= 0); // precondition: n is non-negative
	if (n <= 0) return; // base case
	int i, j;
	for (i = n - 1; i > 0; i--) {
		assert(0 <= i && i <= n-1); // loop invariant: i is between 0 and n-1
		for (int k = 0; k < i; k++) { // loop invariant: the elements of the array from index 0 to index i are sorted in ascending order
			assert(array[k] <= array[k+1]);
		}
		for (j = 0; j < i; j++) {
			assert(0 <= j && j <= i); // loop invariant: j is between 0 and i
			for (int k = 0; k < j; k++) { // loop invariant: the elements of the array from index 0 to index j are sorted in ascending order
				assert(array[k] <= array[k+1]);
			}
			for (int k = j+1; k < n; k++) { // loop invariant: the element at index j is less than or equal to all the elements from index j+1 to index n-1
				assert(array[j] <= array[k]);
			}
			if (array[j] > array[j+1]) {
				swap(&array[j], &array[j+1]);
			}
		}
	}
	for (int i = 0; i < n-1; i++) { // postcondition: array is sorted in ascending order
		assert(array[i] <= array[i+1]);
	}
}

void main() {
	int array [N] = {10, 7, 9, ...};
	bubbleSort(array, N);
}


==> Code/infill.tex <==
void bubbleSort(int *array, int n) {
    int i, j;
    for(i = n - 1; i > 0; i--) {
        /* @ >>> INFILL <<< */
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

==> Code/moti.tex <==
#include <limits.h>

/*@
requires \valid(a);
requires \valid(b);
ensures *a == \old(*b);
ensures *b == \old(*a);
assigns *a,*b;
*/
void swap(int *a, int *b) {
    int temp = *a;
    *a = *b;
    *b = temp;
}

/*@ 
requires \valid(array+(0..n-1));
requires 0 < n < INT_MAX;
ensures \forall integer i; 0 < i < n ==> array[i-1] <= array[i];
*/
void bubbleSort(int *array, int n) {
    if (n <= 0) return;
    int i, j;
    /*@
    loop invariant 0 <= i < n;
    loop invariant \forall integer k; i <= k < n-1 ==> array[k] <= array[k+1];
    loop invariant \forall integer k; 0 <= k < i+1 <= n-1 ==> array[k] <= array[i+1];
    loop assigns i, j, array[0..n-1];
    */
    for(i = n - 1; i > 0; i--) {
        /*@
        loop invariant 0 <= j <= i < n;
        loop invariant \forall integer k; 0 <= k <= j ==> array[k] <= array[j];
        loop invariant \forall integer k; 0 <= k < i+1 <= n-1 ==> array[k] <= array[i+1];
        loop assigns j, array[0..i];
        */
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

void main() {
    int array[5000] = {..., 5, 4, 3, 2, 1};
    bubbleSort(array, 5000);
    //@ assert \forall int i; 0 < i < 5000 ==> array[i-1] <= array[i];
}

==> Code/source-code.tex <==
void swap(int *a, int *b) {
    int temp = *a;
    *a = *b;
    *b = temp;
}

void bubbleSort(int *array, int n) {
    if (n <= 0) return;
    int i, j;
    for(i = n - 1; i > 0; i--) {
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

void main() {
    int array[5000] = {..., 5, 4, 3, 2, 1};
    bubbleSort(array, 5000);
    //@ assert \forall int i; 0 < i < 5000 ==> array[i-1] <= array[i];
}

==> FigureTex/figure-passk.tex <==
\begin{figure*}[ht]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\textwidth]{./Figure/rq-passk.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Pass@K on Code Completion Over Years}
    \label{fig:passk}
\end{figure*} 

==> FigureTex/figure-rq123-design.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\linewidth]{./Figure/design-123-3.pdf}
    % \setlength{\abovecaptionskip}{-5pt}
    % \setlength{\belowcaptionskip}{-5pt}
    \caption{\textbf{Experiment Design for RQ1-3.} We assess LLMs' performance on contaminated/fresh data. Three countermeasures (\ie, using newly-\textbf{collected}/ \textbf{constructed}/ \textbf{refactored} data) are considered.}
    \label{fig:rq123-design}
\end{figure} 

==> FigureTex/figure-sim-design.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=0.75\linewidth]{./Figure/design-sim.pdf}
    % \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-15pt}
    \caption{Pairwise Code Similarity Comparison}
    \label{fig:simi}
\end{figure} 

==> FigureTex/figure-similarity-heatmap.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=0.85\linewidth]{./Figure/rq-similarity-all.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Code Similarities Over Various Code Groups}
    \label{fig:rq-sim}
\end{figure} 

==> FigureTex/figure_pass1.tex <==
\begin{figure*}[th]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=0.9\textwidth]{./Figure/rq-full.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Overall Comparison on Pass@1 of RQ1-3 
    % \wac{Need to separate if and while. And we don't need to distinguish refactor and new refactor.}
    }
    \label{fig:pass-all}
\end{figure*}

==> FigureTex/figure_refactor_complexity.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=0.85\linewidth]{./Figure/complexity.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Complexity Comparison of Various Code Groups
    % \wac{Do we still include this?}
    }
    \label{fig:refactor-complex}
\end{figure} 

==> FigureTex/ppl_scores.tex <==
\begin{figure*}[t!]
    \centering
    % \vspace{-0ex}
    % \begin{subfigure}[b]{1.0\textwidth}
    % \caption{Leakage-related Scores Over Various Code Groups (StarCoder)}
    \includegraphics[width=0.95\textwidth]{./Figure/rq-ppl-score-starcoder-instruct.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-30pt}
    % \label{fig:rq-score-star}
    % \end{subfigure}

    % \begin{subfigure}[b]{1.0\textwidth}
    % \caption{Leakage-related Scores Over Various Code Groups (WizardCoder)}
    % \includegraphics[width=1.0\textwidth]{../Figure/rq-ppl-score-wizardCoder.png}
    % \setlength{\abovecaptionskip}{-0pt}
    % \setlength{\belowcaptionskip}{-0pt}
    % \label{fig:rq-score-wizard}
    % \end{subfigure}
    
\setlength{\abovecaptionskip}{-0pt}
\setlength{\belowcaptionskip}{-5pt}
\caption{Contamination-related Scores Over Various Code Groups}
\label{fig:rq-score}
\end{figure*} 

==> FigureTex/ppl_scores_rq23.tex <==
\begin{figure*}[ht]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\textwidth]{./Figure/rq-ppl-score-2.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Scores on Benchmarks and Refactored Code}
    \label{fig:rq-score-2}
\end{figure*} 

==> FigureTex/workflow.tex <==
\begin{figure*}[t]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\linewidth]{./Figure/workflow.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Workflow (Draft)}
    \label{fig:workflow}
\end{figure*} 

==> Listing/Listing-case1.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
\label{listing:case1}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            % aboveskip=-8pt,
            % belowskip=-10pt,
		label={listing:case1},
		escapechar=|,
            captionpos=none,
		linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/case-spurious.tex}
\end{figure}

==> Listing/Listing-case2.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
% \label{listing:case2}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            % aboveskip=-8pt,
            belowskip=-8pt,
		label={listing:case2},
		escapechar=|,
            captionpos=none,
		linebackgroundcolor = {\ifnum \value{lstnumber} > 5 \ifnum \value{lstnumber} < 7 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/case-study2.tex}
\end{figure}

==> Listing/Listing-case3.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
% \label{listing:case3}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            aboveskip=-2pt,
            belowskip=-5pt,
		label={listing:case3},
		escapechar=|,
            captionpos=none,
		linebackgroundcolor = {\ifnum \value{lstnumber} > 3 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/case-study3.tex}
\end{figure}

==> Listing/Listing-moti.tex <==
% \begin{figure} [t]
%     \centering
%     \vspace{-0ex}
%     \includegraphics[width=0.7\linewidth]{Figure/moti.pdf}
%     \setlength{\abovecaptionskip}{-0pt}
%     \setlength{\belowcaptionskip}{-0pt}
%     \caption{ACSL annotations to functional proof of the bubble sort}
%     \label{fig:moti}
% \end{figure}

% \begin{listing}[ht]
% \inputminted[
% frame=lines,
% framesep=1mm,
% baselinestretch=1.0,
% fontsize=\footnotesize,
% linenos,
% xleftmargin=5.5ex,
% baselinestretch=1.0,
% ]{c}{../Code/moti.c}
% \caption{ACSL annotations to functional proof of the bubble sort}
% \label{fig:moti}
% \end{listing}

% \setlength{\textfloatsep}{10pt}
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[t]
	\lstinputlisting[
		language=c,
        % basicstyle=\linespread{0.8}\tiny,
            % baselinestretch=1.0,
		% morekeywords={var},
            aboveskip=-8pt,
            belowskip=-20pt,
		caption={\textbf{ACSL Annotations to Functional Proof of {Bubble Sort}}},
		label={fig:moti},
		escapechar=|,
		% linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 10 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/moti.tex}
\end{figure}

==> Listing/listing-temp1.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
\label{listing:case1}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            % aboveskip=-8pt,
            % belowskip=-10pt,
		label={listing:case1},
		escapechar=|,
            captionpos=none,
		% linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/code-temp.tex}
\end{figure}

==> Listing/listing-temp2.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
\label{listing:case1}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            % aboveskip=-8pt,
            % belowskip=-10pt,
		label={listing:case1},
		escapechar=|,
            captionpos=none,
		% linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/code-temp2.tex}
\end{figure}

==> Table/design.tex <==
\begin{table*}[t!]
    \centering
    \renewcommand\arraystretch{1.5}
    \caption{Large Language Models and Datasets}\label{tab:model}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|l|l|r|r|l|l|l}
    \toprule
    \multicolumn{8}{c}{\textbf{Code Large Language Models Statistics}} \\ 
    \midrule

    \multicolumn{5}{c}{\textbf{Model Information}} & \multicolumn{3}{|c}{\textbf{Data Information}} \\ \midrule
    \textbf{Index} & \textbf{Base Model} & \multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{Size}} & \textbf{1st Release} & \multicolumn{1}{c}{\textbf{Source}} & \multicolumn{1}{|c}{\textbf{Time Span}}  & \multicolumn{1}{|c}{\textbf{Programming Languages}} \\ 
    \midrule
    
    {\large \ding{202}} & \multirow{-1}{*}{\textbf{StarCoder}} & \textbf{StarCoder} & 15.5B & May 2023 & the Stack~\cite{Kocetkov2022TheStack} & Jan 2015$\sim$ Mar 2022  & 358 Programming languages \\
    
    {\large \ding{203}} &  & \textbf{StarChat} & 15.5B & Jun 2023 & GitHub & Up to April 2023 & \begin{tabular}[l]{@{}l@{}}80+ programming languages.\end{tabular} \\ 
    
    {\large \ding{204}} & & \textbf{WizardCoder} & 15.5B & Jun 2023 & the Stack~\cite{Kocetkov2022TheStack}, CodeAlpaca-20k & Jan 2015$\sim$ Mar 2023  & 358 Programming languages \\
    \hline
    
    {\large \ding{205}} & & \textbf{CodeLlama-Instruct} & 7B  & Apr 2023 & GitHub + StackOverflow & Up to Jan 2023 & \begin{tabular}[l]{@{}c@{}}Python, C/C++, TypeScript, Java, \etc \end{tabular} \\
     
    {\large \ding{206}} & \multirow{-2}{*}{\textbf{Llama2}} & \textbf{Phind-CodeLlama} & 34B & Aug 2023 & GitHub + StackOverflow & Up to Aug 2023 & \begin{tabular}[l]{@{}c@{}}Python, C/C++, TypeScript, Java, \etc \end{tabular} \\
    \hline
    
    % \textbf{Dense} & \textbf{InCoder} & 1B  & Apr 2022 & GitHub, GitLab, StackOverflow & Up to Apr 2022 & Python, JavaScript and 28 languages \\ 
    
    % \hline
    % \textbf{SantaCoder} & \textbf{SantaCoder} & 1.1B & Dec 2022 & the Stack~\cite{Kocetkov2022TheStack} & Jan 2015$\sim$ Mar 2022 & Python, Java, JavaScript \\

    \hline
    {\large \ding{207}} & \textbf{GLM} & \textbf{ChatGLM2} & 6B & Oct 2023 & -- & Up to May 2022  & Python, Java, JavaScript \\
    
    \hline
    {\large \ding{208}} & & \textbf{ChatGPT 3.5-turbo} & -- & June 2023 & Public Data & Up to Sep 2021  & 95+ Programming languages \\
     
    {\large \ding{209}} & \multirow{-2}{*}{\textbf{ChatGPT}} & \textbf{Github-Copilot} & -- & Jun 2021 & Public Data & Up to April 2023  & 95+ Programming languages \\
\bottomrule
    \end{tabular}
    }
\end{table*}

==> Table/java-modelwise.tex <==

\begin{table}[b!]
\centering
\renewcommand\arraystretch{1.2}
\caption{\textbf{RQ4: Model-wise Effectiveness of 4 Operators on Method-level Java Code.} The \colorbox[HTML]{95B0E7}{bluer}, the better. (Metrics: Min\_20\% Prob)}
\label{tab:rq4}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l||cc||c||c}
\toprule
 & \multicolumn{2}{c||}{Syntactic} & \multicolumn{1}{c||}{Semantic} & Style \\
 \hline
Models  & IFF & Loop & Renm & Norm \\ 
 \midrule
 

Starcoder & 8.083 & \cellcolor[HTML]{F3F7FD}0.051 & \cellcolor[HTML]{DCE6F9}0.145 & \cellcolor[HTML]{FAC1CE}-0.026 \\
CodeLlama & \cellcolor[HTML]{D7E2F8}0.167 & \cellcolor[HTML]{F2F6FD}0.056 & \cellcolor[HTML]{96B0E7}2.22E+38 & \cellcolor[HTML]{FCFDFF}0.016 \\
WizardCoder & 0.221 & \cellcolor[HTML]{D0DDF6}8.699 & \cellcolor[HTML]{DAE5F8}0.153 & \cellcolor[HTML]{FCDDE3}-0.019 \\
Starchat & 7.196 & \cellcolor[HTML]{F2F6FD}0.055 & \cellcolor[HTML]{DEE7F9}0.139 & \cellcolor[HTML]{FDEFF2}-0.014 \\

\midrule
Average & 3.917 & \cellcolor[HTML]{D0DDF6}2.215 & \cellcolor[HTML]{C2D2F3}5.54E+37 & \cellcolor[HTML]{FFFFFF}-0.011

 \\
\bottomrule
\end{tabular}
}
\end{table}




==> Table/rq1-pass1-1.tex <==

\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.2}
\caption{\textbf{Pass@1 with Nucleus Sampling on Contaminated/Collected/Crafted Code Groups.}
The \colorbox[HTML]{97C3C2}{greener}, the larger. 
We \textbf{\underline{underline}} the results on the data collected \textit{after}
each model's release time (\ie, {{fresh}}) to facilitate clearer demonstration.
% The \colorbox{nord9}{bluer}, the smaller, while the \colorbox{nord11}{redder}, the larger. The white is in between.
}
\label{tab:rq1}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccc||cc||cc}
\toprule
                    & \multicolumn{1}{c}{\textbf{Code-2018}} & \multicolumn{1}{c}{\textbf{Code-2019}} & \multicolumn{1}{c}{\textbf{Code-2020}} & \multicolumn{1}{c}{\textbf{Code-2021}} & \multicolumn{1}{c||}{\textbf{Code-2022}} & \multicolumn{1}{c}{\textbf{Code-2023}} & \multicolumn{1}{c||}{\textbf{Code-2023-oct}} & \multicolumn{1}{c}{\textbf{Code-HumE}} & \multicolumn{1}{c}{\textbf{Code-CodE}} \\
\cline{2-10}
\textbf{Model}      & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c||}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c||}{Pass@1}            & \multicolumn{1}{c}{Pass@1}             & \multicolumn{1}{c}{Pass@1}             \\
\midrule
\textbf{StarCoder} & \cellcolor[HTML]{E7F1F1}30.8 & \cellcolor[HTML]{E8F2F2}30.5 & \cellcolor[HTML]{E9F2F2}30.2 & \cellcolor[HTML]{EBF3F3}29.4 & \cellcolor[HTML]{F0F7F7}27.3 & \cellcolor[HTML]{DEECEC}\underline{34.1} & \cellcolor[HTML]{DFEDED}\underline{33.9} & \cellcolor[HTML]{CDE2E2}\underline{40.9} & \cellcolor[HTML]{B2D2D2}51.2 \\
\textbf{StarChat} & \cellcolor[HTML]{D6E7E7}37.2 & \cellcolor[HTML]{DEECEC}34.4 & \cellcolor[HTML]{DAEAEA}35.7 & \cellcolor[HTML]{D3E6E6}38.5 & \cellcolor[HTML]{E2EEEE}32.6 & \cellcolor[HTML]{D1E4E4}39.3 & \cellcolor[HTML]{CAE0E0}\underline{41.9} & \cellcolor[HTML]{B8D6D6}48.7 & \cellcolor[HTML]{B8D6D6}48.8 \\
\textbf{WizardCoder} & \cellcolor[HTML]{D3E6E6}38.5 & \cellcolor[HTML]{DCEBEB}34.9 & \cellcolor[HTML]{D3E6E6}38.5 & \cellcolor[HTML]{CEE3E3}40.4 & \cellcolor[HTML]{DEECEC}34.1 & \cellcolor[HTML]{CDE2E2}40.6 & \cellcolor[HTML]{C5DDDD}\underline{43.8} & \cellcolor[HTML]{AFD1D1}52.2 & \cellcolor[HTML]{A7CCCC}55.5 \\
\textbf{CodeLlama} & \cellcolor[HTML]{D7E8E8}37.0 & \cellcolor[HTML]{D6E7E7}37.2 & \cellcolor[HTML]{D7E8E8}37.0 & \cellcolor[HTML]{D3E6E6}38.5 & \cellcolor[HTML]{E0EDED}33.6 & \cellcolor[HTML]{D4E6E6}\underline{38.0} & \cellcolor[HTML]{C7DEDE}\underline{43.2} & \cellcolor[HTML]{AFD1D1}52.2 & \cellcolor[HTML]{A7CCCC}55.5 \\
\textbf{Phind} & \cellcolor[HTML]{CBE1E1}41.4 & \cellcolor[HTML]{CDE2E2}40.9 & \cellcolor[HTML]{C5DDDD}44.0 & \cellcolor[HTML]{C4DDDD}44.3 & \cellcolor[HTML]{D2E5E5}38.8 & \cellcolor[HTML]{D4E6E6}38.0 & \cellcolor[HTML]{BEDADA}\underline{46.4} & \cellcolor[HTML]{98C3C3}60.9 & \cellcolor[HTML]{A5CBCB}56.1 \\
\textbf{ChatGLM2} & \cellcolor[HTML]{FCFEFE}22.7 & \cellcolor[HTML]{F8FBFB}24.2 & \cellcolor[HTML]{F8FBFB}24.2 & \cellcolor[HTML]{FFFFFF}21.4 & \cellcolor[HTML]{FEFEFE}22.1 & \cellcolor[HTML]{FCFEFE}\underline{22.7} & \cellcolor[HTML]{F0F7F7}\underline{27.3} & \cellcolor[HTML]{E7F1F1}\underline{30.9} & \cellcolor[HTML]{DDEBEB}34.8 \\
\textbf{gpt-3.5} & \cellcolor[HTML]{E3EFEF}32.3 & \cellcolor[HTML]{E9F2F2}30.2 & \cellcolor[HTML]{E7F1F1}30.7 & \cellcolor[HTML]{E4F0F0}31.8 & \cellcolor[HTML]{EEF5F5}\underline{28.1} & \cellcolor[HTML]{DEECEC}\underline{34.1} & \cellcolor[HTML]{D6E7E7}\underline{37.5} & \cellcolor[HTML]{BCD8D8}\underline{47.4} & \cellcolor[HTML]{B0D1D1}51.8 \\
\textbf{Copilot} & \cellcolor[HTML]{B9D6D6}48.4 & \cellcolor[HTML]{B8D6D6}49.0 & \cellcolor[HTML]{B8D6D6}48.7 & \cellcolor[HTML]{ACCFCF}53.4 & \cellcolor[HTML]{C2DCDC}44.8 & \cellcolor[HTML]{B4D3D3}50.5 & \cellcolor[HTML]{A5CBCB}\underline{56.0} & \cellcolor[HTML]{9BC5C5}60.0 & \cellcolor[HTML]{A0C8C8}57.9

 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Table/rq1-pass1.tex <==
\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.3}
\caption{\textbf{Pass@1 with Nucleus Sampling on Contaminated/Collected/Crafted Code Groups.}
The \colorbox[HTML]{97C3C2}{greener}, the larger. 
We \textbf{\underline{underline}} the results on the data collected \textit{after}
each model's release time (\ie, {{fresh}}) to facilitate clearer demonstration.
% The \colorbox{nord9}{bluer}, the smaller, while the \colorbox{nord11}{redder}, the larger. The white is in between.
}
\label{tab:rq1}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccc||cc||cc}
\toprule
                    & \multicolumn{1}{c}{\textbf{Code-2018}} & \multicolumn{1}{c}{\textbf{Code-2019}} & \multicolumn{1}{c}{\textbf{Code-2020}} & \multicolumn{1}{c}{\textbf{Code-2021}} & \multicolumn{1}{c||}{\textbf{Code-2022}} & \multicolumn{1}{c}{\textbf{Code-2023}} & \multicolumn{1}{c||}{\textbf{Code-2023-oct}} & \multicolumn{1}{c}{\textbf{Code-CodE}} & \multicolumn{1}{c}{\textbf{Code-HumE}} \\
\cline{2-10}
\textbf{Model}      & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c||}{Pass@1}        & \multicolumn{1}{c}{Pass@1}        & \multicolumn{1}{c||}{Pass@1}            & \multicolumn{1}{c}{Pass@1}             & \multicolumn{1}{c}{Pass@1}             \\
\midrule
\textbf{Starcode}   & \cellcolor[HTML]{EDF5F5}27.3      & \cellcolor[HTML]{EDF5F5}27.1      & \cellcolor[HTML]{EEF6F6}26.6      & \cellcolor[HTML]{EBF4F4}27.9      & \cellcolor[HTML]{EEF6F6}26.6      & \multicolumn{1}{c}{\cellcolor[HTML]{DFEDED}{\underline{32.6}}}      & \cellcolor[HTML]{DFEDED}{\underline{32.8}}          & \cellcolor[HTML]{CBE1E1}{\underline{40.9}}           & \cellcolor[HTML]{DDEBEB}{{33.5}}           \\ 


\textbf{StarChat}   & \cellcolor[HTML]{DCEBEB}33.9      & \cellcolor[HTML]{E3EFEF}31.0      & \cellcolor[HTML]{E0EDED}32.3      & \cellcolor[HTML]{D4E6E6}37.2      & \cellcolor[HTML]{E3EFEF}31.2      & \cellcolor[HTML]{D4E6E6}37.0      & \cellcolor[HTML]{CBE1E1}{\underline{40.9}}          & \cellcolor[HTML]{B7D5D5}\underline{48.7}           & \cellcolor[HTML]{DFECEC}{32.9}           \\

\textbf{Codellama}  & \cellcolor[HTML]{DCEBEB}33.9      & \cellcolor[HTML]{DCEBEB}34.1      & \cellcolor[HTML]{DCEBEB}33.9      & \cellcolor[HTML]{D4E6E6}37.0      & \cellcolor[HTML]{E0EDED}32.3      & \cellcolor[HTML]{D6E8E8}\underline{36.2}      & \cellcolor[HTML]{C7DFDF}\underline{42.2}          & \cellcolor[HTML]{AED0D0}52.2           & \cellcolor[HTML]{DAEAEA}34.8           \\

\textbf{WizardCoder} & \cellcolor[HTML]{DAE9E9}34.9      & \cellcolor[HTML]{E0EDED}32.3      & \cellcolor[HTML]{D9E9E9}35.2      & \cellcolor[HTML]{D0E4E4}38.8      & \cellcolor[HTML]{DEECEC}33.1      & \cellcolor[HTML]{D0E4E4}38.8      & \cellcolor[HTML]{C6DEDE}\underline{42.7}          & \cellcolor[HTML]{AED0D0}52.2           & \cellcolor[HTML]{CBE1E1}40.9           \\

\textbf{Phind}      & \cellcolor[HTML]{D2E5E5}38.0      & \cellcolor[HTML]{D1E4E4}38.3      & \cellcolor[HTML]{CCE1E1}40.4      & \cellcolor[HTML]{C5DDDD}43.2      & \cellcolor[HTML]{D2E5E5}37.8      & \cellcolor[HTML]{D3E6E6}37.5      & \cellcolor[HTML]{C0DADA}\underline{45.3}          & \cellcolor[HTML]{98C3C3}60.9           & \cellcolor[HTML]{CBE1E1}40.9           \\

\textbf{Chatglm2}   & \cellcolor[HTML]{FFFFFF}19.8      & \cellcolor[HTML]{FCFEFE}21.1      & \cellcolor[HTML]{FCFEFE}21.1      & \cellcolor[HTML]{FFFFFF}19.8      & \cellcolor[HTML]{FDFEFE}20.6      & \cellcolor[HTML]{FCFEFE}21.1      & \cellcolor[HTML]{EFF6F6}\underline{26.3}          & \cellcolor[HTML]{E4EFEF}30.9           & \cellcolor[HTML]{F7FBFB}23.2           \\

\textbf{gpt-3.5}    & \cellcolor[HTML]{E8F2F2}29.2      & \cellcolor[HTML]{EBF3F3}28.1      & \cellcolor[HTML]{ECF4F4}27.6      & \cellcolor[HTML]{E5F0F0}30.2      & \cellcolor[HTML]{EEF5F5}\underline{26.8}      & \cellcolor[HTML]{DFEDED}\underline{32.6}      & \cellcolor[HTML]{D6E8E8}\underline{36.2}          & \cellcolor[HTML]{BAD7D7}\underline{47.4}           & \cellcolor[HTML]{D5E7E7}\underline{36.6}           \\

\textbf{Copilot}    & \cellcolor[HTML]{C1DBDB}44.8      & \cellcolor[HTML]{BDD9D9}46.4      & \cellcolor[HTML]{BFDADA}45.6      & \cellcolor[HTML]{ADCFCF}52.9      & \cellcolor[HTML]{C3DCDC}43.8      & \cellcolor[HTML]{B8D6D6}48.2      & \cellcolor[HTML]{A6CBCB}\underline{55.5}          & \cellcolor[HTML]{9BC5C5}\underline{60.0}           & \cellcolor[HTML]{CFE3E3}\underline{39.0}          

 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Table/rq1-pass5-1.tex <==
\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.2}
\caption{\textbf{Pass@5 with Nucleus Sampling on Contaminated/Collected/Crafted Code Groups.}
The \colorbox[HTML]{97C3C2}{greener}, the larger. 
We \textbf{\underline{underline}} the results on the data collected \textit{after}
each model's release time (\ie, {{fresh}}) to facilitate clearer demonstration.
% The \colorbox{nord9}{bluer}, the smaller, while the \colorbox{nord11}{redder}, the larger. The white is in between.
}
\label{tab:rq1-p5}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccc||cc||cc}
\toprule
                    & \multicolumn{1}{c}{\textbf{Code-2018}} & \multicolumn{1}{c}{\textbf{Code-2019}} & \multicolumn{1}{c}{\textbf{Code-2020}} & \multicolumn{1}{c}{\textbf{Code-2021}} & \multicolumn{1}{c||}{\textbf{Code-2022}} & \multicolumn{1}{c}{\textbf{Code-2023}} & \multicolumn{1}{c||}{\textbf{Code-2023-oct}} & \multicolumn{1}{c}{\textbf{Code-HumE}} & \multicolumn{1}{c}{\textbf{Code-CodE}} \\
\cline{2-10}
\textbf{Model}      & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c||}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c||}{Pass@5}            & \multicolumn{1}{c}{Pass@5}             & \multicolumn{1}{c}{Pass@5}             \\
\midrule

\textbf{StarCoder} & \cellcolor[HTML]{E9F3F3}33.6 & \cellcolor[HTML]{EBF4F4}32.8 & \cellcolor[HTML]{EBF3F3}33.1 & \cellcolor[HTML]{EFF6F6}31.2 & \cellcolor[HTML]{FAFCFC}27.3 & \cellcolor[HTML]{E2EEEE}\underline{36.5} & \cellcolor[HTML]{DEECEC}\underline{37.8} & \cellcolor[HTML]{D2E5E5}\underline{42.6} & \cellcolor[HTML]{B2D2D2}54.9 \\
\textbf{StarChat} & \cellcolor[HTML]{D7E8E8}40.6 & \cellcolor[HTML]{DEECEC}38.0 & \cellcolor[HTML]{DAE9E9}39.6 & \cellcolor[HTML]{D3E6E6}42.2 & \cellcolor[HTML]{E0EDED}37.2 & \cellcolor[HTML]{D4E6E6}41.7 & \cellcolor[HTML]{D4E6E6}\underline{41.9} & \cellcolor[HTML]{B6D5D5}53.5 & \cellcolor[HTML]{B2D2D2}54.9 \\
\textbf{WizardCoder} & \cellcolor[HTML]{D6E8E8}40.9 & \cellcolor[HTML]{DEECEC}37.8 & \cellcolor[HTML]{D6E8E8}40.9 & \cellcolor[HTML]{CFE3E3}43.8 & \cellcolor[HTML]{E0EDED}37.2 & \cellcolor[HTML]{D2E5E5}42.4 & \cellcolor[HTML]{C3DCDC}\underline{48.4} & \cellcolor[HTML]{A9CDCD}58.3 & \cellcolor[HTML]{AACECE}57.9 \\
\textbf{CodeLlama} & \cellcolor[HTML]{D7E8E8}40.6 & \cellcolor[HTML]{D8E9E9}40.1 & \cellcolor[HTML]{D6E7E7}41.1 & \cellcolor[HTML]{D6E7E7}41.1 & \cellcolor[HTML]{E0EDED}37.0 & \cellcolor[HTML]{D6E7E7}\underline{41.4} & \cellcolor[HTML]{C8DFDF}\underline{46.6} & \cellcolor[HTML]{ADCFCF}57.0 & \cellcolor[HTML]{B2D2D2}54.9 \\
\textbf{Phind} & \cellcolor[HTML]{CFE3E3}43.8 & \cellcolor[HTML]{CEE3E3}44.0 & \cellcolor[HTML]{C8DFDF}46.4 & \cellcolor[HTML]{C6DEDE}47.4 & \cellcolor[HTML]{D2E5E5}42.4 & \cellcolor[HTML]{DAE9E9}39.6 & \cellcolor[HTML]{C6DEDE}\underline{47.4} & \cellcolor[HTML]{A2C9C9}61.3 & \cellcolor[HTML]{AACECE}57.9 \\
\textbf{ChatGLM2} & \cellcolor[HTML]{ECF4F4}32.6 & \cellcolor[HTML]{FAFCFC}27.3 & \cellcolor[HTML]{F9FCFC}27.6 & \cellcolor[HTML]{FEFFFF}25.5 & \cellcolor[HTML]{FFFFFF}25.0 & \cellcolor[HTML]{FBFDFD}\underline{26.8} & \cellcolor[HTML]{F1F7F7}\underline{30.5} & \cellcolor[HTML]{E6F1F1}\underline{34.8} & \cellcolor[HTML]{E0EDED}37.2 \\
\textbf{gpt-3.5} & \cellcolor[HTML]{E7F1F1}34.4 & \cellcolor[HTML]{ECF4F4}32.6 & \cellcolor[HTML]{EFF6F6}31.2 & \cellcolor[HTML]{E8F2F2}33.9 & \cellcolor[HTML]{F2F8F8}30.2 & \cellcolor[HTML]{E5F0F0}\underline{35.4} & \cellcolor[HTML]{D9E9E9}\underline{39.8} & \cellcolor[HTML]{C1DBDB}\underline{49.1} & \cellcolor[HTML]{B1D2D2}55.5 \\
\textbf{Copilot} & \cellcolor[HTML]{BED9D9}50.5 & \cellcolor[HTML]{BED9D9}50.3 & \cellcolor[HTML]{BBD7D7}51.6 & \cellcolor[HTML]{AFD0D0}56.2 & \cellcolor[HTML]{C8DFDF}46.6 & \cellcolor[HTML]{BED9D9}50.5 & \cellcolor[HTML]{A8CCCC}\underline{58.9} & \cellcolor[HTML]{98C3C3}64.8 & \cellcolor[HTML]{9FC7C7}62.2
  


 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Table/rq1-pass5.tex <==
\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.3}
\caption{\textbf{Pass@5 with Nucleus Sampling on Contaminated/Collected/Crafted Code Groups.}
The \colorbox[HTML]{97C3C2}{greener}, the larger. 
We \textbf{\underline{underline}} the results on the data collected \textit{after}
each model's release time (\ie, {{fresh}}) to facilitate clearer demonstration.
% The \colorbox{nord9}{bluer}, the smaller, while the \colorbox{nord11}{redder}, the larger. The white is in between.
}
\label{tab:rq1-p5}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccc||cc||cc}
\toprule
                    & \multicolumn{1}{c}{\textbf{Code-2018}} & \multicolumn{1}{c}{\textbf{Code-2019}} & \multicolumn{1}{c}{\textbf{Code-2020}} & \multicolumn{1}{c}{\textbf{Code-2021}} & \multicolumn{1}{c||}{\textbf{Code-2022}} & \multicolumn{1}{c}{\textbf{Code-2023}} & \multicolumn{1}{c||}{\textbf{Code-2023-oct}} & \multicolumn{1}{c}{\textbf{Code-CodE}} & \multicolumn{1}{c}{\textbf{Code-HumE}} \\
\cline{2-10}
\textbf{Model}      & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c||}{Pass@5}        & \multicolumn{1}{c}{Pass@5}        & \multicolumn{1}{c||}{Pass@5}            & \multicolumn{1}{c}{Pass@5}             & \multicolumn{1}{c}{Pass@5}             \\
\midrule

\textbf{Starcode}       & \cellcolor[HTML]{EEF5F5}29.9           & \cellcolor[HTML]{EFF6F6}29.7           & \cellcolor[HTML]{F0F6F6}29.4           & \cellcolor[HTML]{EFF6F6}29.7           & \cellcolor[HTML]{F0F6F6}29.4           & \cellcolor[HTML]{E2EEEE}\underline{34.9}           & \cellcolor[HTML]{DEECEC}\underline{36.7}               & \cellcolor[HTML]{CFE3E3}42.6           & \cellcolor[HTML]{DCEBEB}37.2           \\
\textbf{StarChat} & \cellcolor[HTML]{DCEBEB}37.2           & \cellcolor[HTML]{E4EFEF}34.1           & \cellcolor[HTML]{DFECEC}36.2           & \cellcolor[HTML]{D4E6E6}40.6           & \cellcolor[HTML]{DFECEC}36.2           & \cellcolor[HTML]{D7E8E8}39.3           & \cellcolor[HTML]{D3E6E6}40.9               & \cellcolor[HTML]{B4D4D4}53.5           & \cellcolor[HTML]{D9E9E9}38.4           \\
\textbf{Codellama}      & \cellcolor[HTML]{DBEAEA}37.8           & \cellcolor[HTML]{DDEBEB}37.0           & \cellcolor[HTML]{DAEAEA}38.0           & \cellcolor[HTML]{D4E6E6}40.4           & \cellcolor[HTML]{E1EEEE}35.4           & \cellcolor[HTML]{D6E8E8}39.6           & \cellcolor[HTML]{C8DFDF}45.6               & \cellcolor[HTML]{ACCFCF}57.0           & \cellcolor[HTML]{D8E8E8}39.0           \\
\textbf{Wizardcode}     & \cellcolor[HTML]{DCEBEB}37.2           & \cellcolor[HTML]{E1EEEE}35.2           & \cellcolor[HTML]{DCEBEB}37.5           & \cellcolor[HTML]{D0E4E4}42.4           & \cellcolor[HTML]{E0EDED}35.9           & \cellcolor[HTML]{D4E6E6}40.6           & \cellcolor[HTML]{C3DCDC}47.4               & \cellcolor[HTML]{A8CDCD}58.3           & \cellcolor[HTML]{CFE3E3}42.7           \\
\textbf{Phind}          & \cellcolor[HTML]{D6E7E7}39.8           & \cellcolor[HTML]{D2E5E5}41.4           & \cellcolor[HTML]{CFE3E3}42.7           & \cellcolor[HTML]{C6DEDE}46.4           & \cellcolor[HTML]{D3E5E5}41.1           & \cellcolor[HTML]{DAE9E9}38.3           & \cellcolor[HTML]{C6DEDE}46.4               & \cellcolor[HTML]{A1C9C9}61.3           & \cellcolor[HTML]{CDE2E2}43.3           \\
\textbf{Chatglm2}       & \cellcolor[HTML]{F0F6F6}29.2           & \cellcolor[HTML]{FCFEFE}24.2           & \cellcolor[HTML]{FCFDFD}24.5           & \cellcolor[HTML]{FDFEFE}24.0           & \cellcolor[HTML]{FFFFFF}22.9           & \cellcolor[HTML]{FAFCFC}25.3           & \cellcolor[HTML]{F0F6F6}29.4               & \cellcolor[HTML]{E2EEEE}34.8           & \cellcolor[HTML]{F9FCFC}25.6           \\
\textbf{gpt-3.5}        & \cellcolor[HTML]{EBF4F4}31.2           & \cellcolor[HTML]{EEF5F5}29.9           & \cellcolor[HTML]{F3F8F8}28.1           & \cellcolor[HTML]{E8F2F2}32.3           & \cellcolor[HTML]{F1F7F7}\underline{28.9}           & \cellcolor[HTML]{E4F0F0}\underline{33.9}           & \cellcolor[HTML]{D9E9E9}\underline{38.5}               & \cellcolor[HTML]{BFDADA}\underline{49.1}           & \cellcolor[HTML]{D2E5E5}\underline{41.5}           \\
\textbf{Copilot}        & \cellcolor[HTML]{C5DDDD}46.9           & \cellcolor[HTML]{C3DCDC}47.7           & \cellcolor[HTML]{BED9D9}49.5           & \cellcolor[HTML]{AFD1D1}55.7           & \cellcolor[HTML]{C8DFDF}45.3           & \cellcolor[HTML]{BBD8D8}50.8           & \cellcolor[HTML]{A9CDCD}58.1               & \cellcolor[HTML]{98C3C3}\underline{64.8}           & \cellcolor[HTML]{D2E5E5}\underline{41.5}          


 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Table/rq1.tex <==
\begin{table*}[t!]
\centering
\renewcommand\arraystretch{1.5}
\caption{\textbf{Pass@k with Nucleus Sampling on Contaminated/Recent/Curated Code Groups.}
The \colorbox[HTML]{97C3C2}{greener}, the larger. 
We \textbf{\underline{underline}} the results on the data collected \textit{after}
each model's release time (\ie, \textbf{\textit{cleansed}}) to facilitate clearer demonstration.
% The \colorbox{nord9}{bluer}, the smaller, while the \colorbox{nord11}{redder}, the larger. The white is in between.
}
\label{tab:rq1}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lrrr|rrr|rrr|rrr|rrr|rrr||rrr||rrr|rrr}
\toprule
 & \multicolumn{3}{c}{\textbf{Code-2018}} & \multicolumn{3}{c}{\textbf{Code-2019}} & \multicolumn{3}{c}{\textbf{Code-2020}} & \multicolumn{3}{c}{\textbf{Code-2021}} & \multicolumn{3}{c}{\textbf{Code-2022}} & \multicolumn{3}{c||}{\textbf{Code-2023}} & \multicolumn{3}{c||}{\textbf{Code-2023-oct}} & \multicolumn{3}{c}{\textbf{Code-CodE}} & \multicolumn{3}{c}{\textbf{Code-HumE}} \\
\hline
\textbf{Model} & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 \\
 \midrule
\textbf{StarCoder} & \cellcolor[HTML]{E7F1F1}30.70 & \cellcolor[HTML]{E2EEEE}32.60 & \cellcolor[HTML]{E0EDED}{33.60} & \cellcolor[HTML]{E8F2F1}30.50 & \cellcolor[HTML]{E4EFEF}32.00 & \cellcolor[HTML]{E2EEEE}32.80 & \cellcolor[HTML]{E9F2F2}30.20 & \cellcolor[HTML]{E6F1F0}31.20 & \cellcolor[HTML]{E1EEED}33.10 & \cellcolor[HTML]{EBF3F3}29.40 & \cellcolor[HTML]{E9F2F2}30.20 & \cellcolor[HTML]{E6F1F0}31.20 & \cellcolor[HTML]{F0F7F6}27.30 & \cellcolor[HTML]{EBF3F3}29.40 & \cellcolor[HTML]{E8F2F1}30.50 & \cellcolor[HTML]{DEECEC}\underline{34.10} & \cellcolor[HTML]{DBEAEA}\underline{35.40} & \cellcolor[HTML]{D8E9E8}\underline{36.50} & \cellcolor[HTML]{DFECEC}\underline{33.90} & \cellcolor[HTML]{D8E8E8}\underline{36.70} & \cellcolor[HTML]{D5E7E6}\underline{37.80} & \cellcolor[HTML]{CDE2E1}\underline{40.90} & \cellcolor[HTML]{CBE1E0}\underline{41.70} & \cellcolor[HTML]{C8DFDF}\underline{42.60} & \cellcolor[HTML]{B2D2D1}51.20 & \cellcolor[HTML]{AACDCD}54.30 & \cellcolor[HTML]{A8CDCC}54.90 \\
\textbf{StarChat} & \cellcolor[HTML]{D6E7E7}37.20 & \cellcolor[HTML]{D0E4E3}39.80 & \cellcolor[HTML]{CEE2E2}40.60 & \cellcolor[HTML]{DEECEB}34.40 & \cellcolor[HTML]{D7E8E7}37.00 & \cellcolor[HTML]{D4E6E6}38.00 & \cellcolor[HTML]{DAEAE9}35.70 & \cellcolor[HTML]{D2E5E5}38.80 & \cellcolor[HTML]{D0E4E3}39.60 & \cellcolor[HTML]{D3E5E5}38.50 & \cellcolor[HTML]{CCE2E1}41.10 & \cellcolor[HTML]{C9E0DF}42.20 & \cellcolor[HTML]{E2EEEE}32.60 & \cellcolor[HTML]{DBEAEA}35.40 & \cellcolor[HTML]{D6E7E7}37.20 & \cellcolor[HTML]{D1E4E4}39.30 & \cellcolor[HTML]{CCE2E1}41.10 & \cellcolor[HTML]{CBE1E0}41.70 & \cellcolor[HTML]{CAE0E0}\underline{41.90} & \cellcolor[HTML]{CAE0E0}\underline{41.90} & \cellcolor[HTML]{CAE0E0}\underline{41.90} & \cellcolor[HTML]{B8D6D5}48.70 & \cellcolor[HTML]{AED0CF}52.60 & \cellcolor[HTML]{ACCFCE}53.50 & \cellcolor[HTML]{B8D6D5}48.80 & \cellcolor[HTML]{A8CDCC}54.90 & \cellcolor[HTML]{A8CDCC}54.90 \\
\textbf{WizardCoder} & \cellcolor[HTML]{D3E5E5}38.50 & \cellcolor[HTML]{D0E4E3}39.60 & \cellcolor[HTML]{CDE2E1}40.90 & \cellcolor[HTML]{DCEBEB}34.90 & \cellcolor[HTML]{D6E7E7}37.50 & \cellcolor[HTML]{D5E7E6}37.80 & \cellcolor[HTML]{D3E5E5}38.50 & \cellcolor[HTML]{CEE3E2}40.40 & \cellcolor[HTML]{CDE2E1}40.90 & \cellcolor[HTML]{CEE3E2}40.40 & \cellcolor[HTML]{C7DEDE}43.20 & \cellcolor[HTML]{C5DDDD}43.80 & \cellcolor[HTML]{DEECEC}34.10 & \cellcolor[HTML]{D9E9E9}36.20 & \cellcolor[HTML]{D6E7E7}37.20 & \cellcolor[HTML]{CEE2E2}40.60 & \cellcolor[HTML]{CAE0E0}41.90 & \cellcolor[HTML]{C9E0DF}42.40 & \cellcolor[HTML]{C5DDDD}\underline{43.80} & \cellcolor[HTML]{BCD8D7}\underline{47.40} & \cellcolor[HTML]{B9D6D6}\underline{48.40} & \cellcolor[HTML]{AFD1D0}52.20 & \cellcolor[HTML]{A4CAC9}56.50 & \cellcolor[HTML]{9FC7C7}58.30 & \cellcolor[HTML]{A7CCCB}55.50 & \cellcolor[HTML]{A2C9C8}57.30 & \cellcolor[HTML]{A0C8C7}57.90 \\
\textbf{Codellama} & \cellcolor[HTML]{D7E8E7}37.00 & \cellcolor[HTML]{D0E4E3}39.60 & \cellcolor[HTML]{CEE2E2}40.60 & \cellcolor[HTML]{D6E7E7}37.20 & \cellcolor[HTML]{D0E4E3}39.80 & \cellcolor[HTML]{CFE3E3}40.10 & \cellcolor[HTML]{D7E8E7}37.00 & \cellcolor[HTML]{CEE2E2}40.60 & \cellcolor[HTML]{CCE2E1}41.10 & \cellcolor[HTML]{D3E5E5}38.50 & \cellcolor[HTML]{CEE2E2}40.60 & \cellcolor[HTML]{CCE2E1}41.10 & \cellcolor[HTML]{E0EDED}33.60 & \cellcolor[HTML]{DAE9E9}35.90 & \cellcolor[HTML]{D7E8E7}37.00 & \cellcolor[HTML]{D4E6E6}\underline{38.00} & \cellcolor[HTML]{CEE3E2}\underline{40.40} & \cellcolor[HTML]{CBE1E1}\underline{41.40} & \cellcolor[HTML]{C7DEDE}\underline{43.20} & \cellcolor[HTML]{BED9D9}\underline{46.40} & \cellcolor[HTML]{BED9D9}\underline{46.60} & \cellcolor[HTML]{AFD1D0}{52.20} & \cellcolor[HTML]{A6CBCB}{55.70} & \cellcolor[HTML]{A3C9C9}{57.00} & \cellcolor[HTML]{ADCFCF}{53.00} & \cellcolor[HTML]{AACDCD}{54.30} & \cellcolor[HTML]{A8CDCC}{54.90} \\
\textbf{Phind} & \cellcolor[HTML]{CBE1E1}41.40 & \cellcolor[HTML]{C8DFDF}42.70 & \cellcolor[HTML]{C5DDDD}43.80 & \cellcolor[HTML]{CDE2E1}40.90 & \cellcolor[HTML]{C6DEDD}43.50 & \cellcolor[HTML]{C5DDDD}44.00 & \cellcolor[HTML]{C5DDDD}44.00 & \cellcolor[HTML]{C0DADA}45.80 & \cellcolor[HTML]{BED9D9}46.40 & \cellcolor[HTML]{C4DDDC}44.30 & \cellcolor[HTML]{BDD9D8}46.90 & \cellcolor[HTML]{BCD8D7}47.40 & \cellcolor[HTML]{D2E5E5}38.80 & \cellcolor[HTML]{CBE1E1}41.40 & \cellcolor[HTML]{C9E0DF}42.40 & \cellcolor[HTML]{D2E5E5}38.80 & \cellcolor[HTML]{D0E4E3}39.60 & \cellcolor[HTML]{D0E4E3}39.60 & \cellcolor[HTML]{BED9D9}\underline{46.40} & \cellcolor[HTML]{BCD8D7}\underline{47.40} & \cellcolor[HTML]{BCD8D7}\underline{47.40} & \cellcolor[HTML]{99C3C3}60.90 & \cellcolor[HTML]{99C3C3}60.90 & \cellcolor[HTML]{98C3C2}61.30 & \cellcolor[HTML]{A5CBCA}56.10 & \cellcolor[HTML]{A2C9C8}57.30 & \cellcolor[HTML]{A0C8C7}57.90 \\
\textbf{ChatGLM2} & \cellcolor[HTML]{FCFEFD}22.70 & \cellcolor[HTML]{EDF5F4}28.60 & \cellcolor[HTML]{E2EEEE}32.60 & \cellcolor[HTML]{F8FBFB}24.20 & \cellcolor[HTML]{F4F9F8}26.00 & \cellcolor[HTML]{F0F7F6}27.30 & \cellcolor[HTML]{F8FBFB}24.20 & \cellcolor[HTML]{F1F7F7}26.80 & \cellcolor[HTML]{EFF6F6}27.60 & \cellcolor[HTML]{FFFFFF}21.40 & \cellcolor[HTML]{F7FAFA}24.70 & \cellcolor[HTML]{F5F9F9}25.50 & \cellcolor[HTML]{FEFEFE}22.10 & \cellcolor[HTML]{F9FCFB}24.00 & \cellcolor[HTML]{F6FAFA}25.00 & \cellcolor[HTML]{FCFEFD}\underline{22.70} & \cellcolor[HTML]{F5FAF9}\underline{25.30} & \cellcolor[HTML]{F1F7F7}\underline{26.80} & \cellcolor[HTML]{F0F7F6}\underline{27.30} & \cellcolor[HTML]{EEF5F5}\underline{28.10} & \cellcolor[HTML]{E8F2F1}\underline{30.50} & \cellcolor[HTML]{E7F1F1}\underline{30.90} & \cellcolor[HTML]{E2EEEE}\underline{32.60} & \cellcolor[HTML]{DDEBEB}\underline{34.80} & \cellcolor[HTML]{DDEBEB}34.80 & \cellcolor[HTML]{D9E9E9}36.00 & \cellcolor[HTML]{D6E7E7}37.20 \\
\textbf{ChatGPT-3.5} & \cellcolor[HTML]{E3EFEF}32.30 & \cellcolor[HTML]{DEECEC}34.10 & \cellcolor[HTML]{DEECEB}34.40 & \cellcolor[HTML]{E9F2F2}30.20 & \cellcolor[HTML]{E4F0EF}31.80 & \cellcolor[HTML]{E2EEEE}32.60 & \cellcolor[HTML]{E7F1F1}30.70 & \cellcolor[HTML]{E7F1F1}31.00 & \cellcolor[HTML]{E6F1F0}31.20 & \cellcolor[HTML]{E4F0EF}31.80 & \cellcolor[HTML]{E1EDED}33.30 & \cellcolor[HTML]{DFECEC}33.90 & \cellcolor[HTML]{EEF5F5}\underline{28.10} & \cellcolor[HTML]{E9F2F2}\underline{30.20} & \cellcolor[HTML]{E9F2F2}\underline{30.20} & \cellcolor[HTML]{DEECEC}\underline{34.10} & \cellcolor[HTML]{DCEBEA}\underline{35.20} & \cellcolor[HTML]{DBEAEA}\underline{35.40} & \cellcolor[HTML]{D6E7E7}\underline{37.50} & \cellcolor[HTML]{D1E5E4}\underline{39.10} & \cellcolor[HTML]{D0E4E3}\underline{39.80} & \cellcolor[HTML]{BCD8D7}\underline{47.40} & \cellcolor[HTML]{B8D6D5}\underline{48.70} & \cellcolor[HTML]{B7D5D5}\underline{49.10} & \cellcolor[HTML]{B0D1D1}51.80 & \cellcolor[HTML]{AACDCD}54.30 & \cellcolor[HTML]{A7CCCB}55.50 \\
\textbf{Copilot} & \cellcolor[HTML]{B9D6D6}48.40 & \cellcolor[HTML]{B6D4D4}49.70 & \cellcolor[HTML]{B4D3D3}50.50 & \cellcolor[HTML]{B8D6D5}49.00 & \cellcolor[HTML]{B6D4D4}49.70 & \cellcolor[HTML]{B4D4D3}50.30 & \cellcolor[HTML]{B8D6D5}48.70 & \cellcolor[HTML]{B3D3D2}50.80 & \cellcolor[HTML]{B1D2D1}51.60 & \cellcolor[HTML]{ACCFCE}53.40 & \cellcolor[HTML]{A7CCCB}55.50 & \cellcolor[HTML]{A5CBCA}56.20 & \cellcolor[HTML]{C3DCDB}44.80 & \cellcolor[HTML]{BFDAD9}46.10 & \cellcolor[HTML]{BED9D9}46.60 & \cellcolor[HTML]{B4D3D3}50.50 & \cellcolor[HTML]{AED0CF}52.60 & \cellcolor[HTML]{ADCFCF}53.10 & \cellcolor[HTML]{A5CBCA}\underline{56.00} & \cellcolor[HTML]{9FC7C7}\underline{58.30} & \cellcolor[HTML]{9EC6C6}\underline{58.90} & \cellcolor[HTML]{9BC5C4}60.00 & \cellcolor[HTML]{93C0BF}63.00 & \cellcolor[HTML]{8EBDBC}64.80 & \cellcolor[HTML]{A0C8C7}57.90 & \cellcolor[HTML]{97C2C1}61.60 & \cellcolor[HTML]{95C1C1}62.20

 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Table/rq3.tex <==
\begin{table}[t]
\centering
\renewcommand\arraystretch{1.2}
\caption{\textbf{Pass@1 Results (Greedy) on Code-2021 and Five Refactored Code Groups.} 
The entries $\Delta$ is the difference between the previous column and the ``Origin'' column. 
Foreground color \down{blue} means decrease and \upp{red} means increase. The background color highlights the Pass@1 scores: the  \colorbox[HTML]{97C3C2}{greener}, the larger. }
\label{tab:rq3}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|r|rr|rr||rr|rr|rr}
\toprule
 & \multicolumn{1}{c|}{\textbf{Code-2021}} & \multicolumn{2}{c}{\textbf{Code-IFF}} & \multicolumn{2}{c||}{\textbf{Code-Loop}} & \multicolumn{2}{c}{\textbf{Code-Renm}} & \multicolumn{2}{c}{\textbf{Code-Param}} & \multicolumn{2}{c}{\textbf{Code-Deco}} \\ \cline{2-12} 
Model & \multicolumn{1}{c|}{{Pass@1}} & \multicolumn{1}{c}{{ {Pass@1}}} & \multicolumn{1}{c}{$\Delta$} & \multicolumn{1}{c}{{ {Pass@1}}} & \multicolumn{1}{c||}{$\Delta$} & \multicolumn{1}{c}{{ {Pass@1}}} & \multicolumn{1}{c}{$\Delta$} & \multicolumn{1}{c}{{ {Pass@1}}} & \multicolumn{1}{c}{$\Delta$} & \multicolumn{1}{c}{{ {Pass@1}}} & \multicolumn{1}{c}{$\Delta$} \\ \hline

Codellama & \cellcolor[HTML]{D0E4E3}38.5 & \cellcolor[HTML]{D9E9E8}35.1 & \down{-3.4} & \cellcolor[HTML]{C8DFDF}41.8 & \upp{3.3} & \cellcolor[HTML]{D1E4E4}38.2 & \down{-0.3} & \cellcolor[HTML]{D3E6E5}37.3 & \down{-1.2} & \cellcolor[HTML]{F6FAFA}23.4 & \down{-15}.1 \\
StarCode & \cellcolor[HTML]{E7F1F1}29.4 & \cellcolor[HTML]{E4EFEF}30.5 & \upp{1.1} & \cellcolor[HTML]{DAEAE9}34.4 & \upp{5.0} & \cellcolor[HTML]{E4EFEF}30.5 & \upp{1.1} & \cellcolor[HTML]{EBF4F4}27.6 & \down{-1.8} & \cellcolor[HTML]{F3F8F8}24.7 & \down{-4.7} \\
StarChat & \cellcolor[HTML]{D0E4E3}38.5 & \cellcolor[HTML]{D0E4E3}38.5 & \equ{0.0} & \cellcolor[HTML]{CCE1E1}40.2 & \upp{1.7} & \cellcolor[HTML]{D4E6E5}37.1 & \down{-1.4} & \cellcolor[HTML]{D5E6E6}36.7 & \down{-1.8} & \cellcolor[HTML]{E4EFEF}30.5 & \down{-8.0} \\
Wizardcode & \cellcolor[HTML]{CBE1E1}40.4 & \cellcolor[HTML]{CFE3E3}39.1 & \down{-1.3} & \cellcolor[HTML]{BAD7D6}47.5 & \upp{7.1} & \cellcolor[HTML]{CBE1E1}40.4 & \equ{0.0} & \cellcolor[HTML]{CCE1E1}40.2 & \down{-0.2} & \cellcolor[HTML]{F3F8F8}24.5 & \down{-15.9} \\
Phind & \cellcolor[HTML]{C2DBDB}44.3 & \cellcolor[HTML]{B8D6D5}48.3 & \upp{4.0} & \cellcolor[HTML]{ADCFCF}52.5 & \upp{8.2} & \cellcolor[HTML]{C4DDDC}43.3 & \down{-1.0} & \cellcolor[HTML]{C6DEDD}42.5 & \down{-1.8} & \cellcolor[HTML]{CFE3E3}39.1 & \down{-5.2} \\
Chatglm2 & \cellcolor[HTML]{FBFDFD}21.4 & \cellcolor[HTML]{FDFEFE}20.7 & \down{-0.7} & \cellcolor[HTML]{F5F9F9}23.8 & \upp{2.4} & \cellcolor[HTML]{FAFCFC}21.8 & \upp{0.4} & \cellcolor[HTML]{FEFEFE}20.2 & \down{-1.2} & \cellcolor[HTML]{FFFFFF}19.5 & \down{-1.9} \\
gpt-3.5 & \cellcolor[HTML]{E1EEED}31.8 & \cellcolor[HTML]{DEECEC}32.8 & \upp{1.0} & \cellcolor[HTML]{D4E6E6}36.9 & \upp{5.1} & \cellcolor[HTML]{DFEDEC}32.4 & \upp{0.6} & \cellcolor[HTML]{E1EEED}31.8 & \equ{0.0} & \cellcolor[HTML]{E7F1F1}29.4 & \down{-2.4} \\
Copilot & \cellcolor[HTML]{ABCECD}53.4 & \cellcolor[HTML]{9FC7C7}58.0 & \upp{4.6} & \cellcolor[HTML]{8EBDBC}64.8 & \upp{11.4} & \cellcolor[HTML]{A2C9C8}57.1 & 3.7 & \cellcolor[HTML]{BDD9D8}46.2 & \down{-7.2} & \cellcolor[HTML]{BDD9D8}46.1 & \down{-7.3}\\
\bottomrule
% \vspace{-10pt}
\end{tabular}
}
\end{table}
